Keyed Non-Parametric Hypothesis Tests

The recent popularity of machine learning calls for a deeper understanding of AI security. Amongst the numerous AI threats published so far, poisoning attacks currently attract considerable attention. In a poisoning attack the opponent partially tampers the dataset used for learning to mislead the classifier during the testing phase. This paper proposes a new protection strategy against poisoning attacks. The technique relies on a new primitive called keyed non-parametric hypothesis tests allowing to evaluate under adversarial conditions the training input's conformance with a previously learned distribution $\mathfrak{D}$. To do so we use a secret key $\kappa$ unknown to the opponent. Keyed non-parametric hypothesis tests differs from classical tests in that the secrecy of $\kappa$ prevents the opponent from misleading the keyed test into concluding that a (significantly) tampered dataset belongs to $\mathfrak{D}$.

==> diagram.tex <==

\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,270.6666564941406); %set diagram left start at 0, and has height of 270.6666564941406

%Flowchart: Process [id:dp8136119114159726] 
\draw   (111.8,8.73) -- (191.8,8.73) -- (191.8,48.47) -- (111.8,48.47) -- cycle ;
%Straight Lines [id:da9303240539038973] 
\draw    (52.15,37.87) -- (109.5,37.74) ;
\draw [shift={(111.5,37.73)}, rotate = 539.87] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da753279089330275] 
\draw    (251.17,38.07) -- (193.67,37.87) ;
\draw [shift={(191.67,37.87)}, rotate = 360.19] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da556621864673619] 
\draw    (122.2,48.62) -- (121.78,78.08) ;


%Straight Lines [id:da37514867569866484] 
\draw    (182.6,48.62) -- (182.18,78.08) ;


%Flowchart: Process [id:dp07612311702497543] 
\draw   (111.5,129) -- (193.5,129) -- (193.5,168.67) -- (111.5,168.67) -- cycle ;
%Straight Lines [id:da6725300398532541] 
\draw    (182.6,99.12) -- (182.21,126.58) ;
\draw [shift={(182.18,128.58)}, rotate = 270.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da14210445956003737] 
\draw    (123.1,98.62) -- (122.71,126.08) ;
\draw [shift={(122.68,128.08)}, rotate = 270.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7476886767596709] 
\draw    (152.1,168.62) -- (151.71,196.08) ;
\draw [shift={(151.68,198.08)}, rotate = 270.81] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Flowchart: Decision [id:dp8966829173827764] 
\draw   (151.68,198.08) -- (186.68,229.87) -- (151.68,261.67) -- (116.68,229.87) -- cycle ;
%Flowchart: Multidocument [id:dp8921829157110368] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (25.48,18.8) -- (57.48,18.8) -- (57.48,44.1) .. controls (37.48,44.1) and (41.48,53.22) .. (25.48,47.32) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (21.48,22.63) -- (53.48,22.63) -- (53.48,47.93) .. controls (33.48,47.93) and (37.48,57.06) .. (21.48,51.15) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (17.48,26.47) -- (49.48,26.47) -- (49.48,51.77) .. controls (29.48,51.77) and (33.48,60.89) .. (17.48,54.99) -- cycle ;
%Flowchart: Multidocument [id:dp9643025357356452] 
\draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (260,18.67) -- (292,18.67) -- (292,43.97) .. controls (272,43.97) and (276,53.09) .. (260,47.19) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (256,22.5) -- (288,22.5) -- (288,47.8) .. controls (268,47.8) and (272,56.92) .. (256,51.02) -- cycle ; \draw  [fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (252,26.33) -- (284,26.33) -- (284,51.63) .. controls (264,51.63) and (268,60.76) .. (252,54.85) -- cycle ;
%Straight Lines [id:da8926176979293821] 
\draw    (224.5,18.67) -- (194.67,18.85) ;
\draw [shift={(192.67,18.87)}, rotate = 359.64] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da2438212838988767] 
\draw    (117.25,230) -- (90.83,229.79) ;
\draw [shift={(88.83,229.78)}, rotate = 360.45] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8734961773527257] 
\draw    (186.68,229.87) -- (210.75,230.3) ;
\draw [shift={(212.75,230.33)}, rotate = 181.01] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


% Text Node
\draw (33.33,40) node [color={rgb, 255:red, 74; green, 144; blue, 226 }  ,opacity=1 ]  {$D'$};
% Text Node
\draw (267,38.5) node [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ]  {$D$};
% Text Node
\draw (151.8,28.6) node [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ]  {$f$};
% Text Node
\draw (233.5,14.5) node [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ]  {$\kappa $};
% Text Node
\draw (184,89) node   {$f_{\kappa }( D)$};
% Text Node
\draw (126,89) node   {$f_{\kappa }( D')$};
% Text Node
\draw (152.5,147.83) node [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,opacity=1 ]  {$\mu $};
% Text Node
\draw (151.68,225.87) node   {$p< \textcolor[rgb]{0.96,0.65,0.14}{\tau }$};
% Text Node
\draw (39.93,228) node  [align=left] {{\fontfamily{pcr}\selectfont reject}};
% Text Node
\draw (230.27,228.33) node  [align=left] {{\fontfamily{pcr}\selectfont use}};
% Text Node
\draw (75.33,227.17) node   {$D'$};
% Text Node
\draw (254.33,227.53) node   {$D'$};
% Text Node
\draw (107,218) node [scale=0.7] [align=left] {{\fontfamily{pcr}\selectfont yes}};


\end{tikzpicture}
